Breaking Writer's Block: Low-cost Fine-tuning of Natural Language Generation Models

It is standard procedure these days to solve Information Extraction task by fine-tuning large pre-trained language models. This is not the case for generation task, which relies on a variety of techniques for controlled language generation. In this paper, we describe a system that fine-tunes a natural language generation model for the problem of solving Writer's Block. The fine-tuning changes the conditioning to also include the right context in addition to the left context, as well as an optional list of entities, the size, the genre and a summary of the paragraph that the human author wishes to generate. Our proposed fine-tuning obtains excellent results, even with a small number of epochs and a total cost of USD 150. The system can be accessed as a web-service, and all the code is released. A video showcasing the interface and the model is also available.

==> _conclu.tex <==
In this paper, we present an end-to-end pipeline from Project Gutenberg library's raw text file to a web-service intended for book writers. The latter embeds a controllable and contextualised GPT-2 for text generation specific to novels. It was fine-tuned following our pipeline on a few hundreds of novels during ten epochs. Despite being limited by the computational resources at our disposal, we demonstrate that our final model is able to take into consideration the context specified by the user. With the constant improvement of computing capacities and recent research trend aimed at reducing model size without damaging generation capacities, we strongly believe such controllable generative framework will be easily accessible in the future and will greatly enhance the creativity of writers. 



%Despite being limited by the computational resources at our disposal, we fine-tune it on a few hundreds of novels during ten epochs, following an innovative approach. Using our pipeline, we fine-tune a small GPT-2 on a few hundreds of novels during ten epochs. while being limited by the computational resources at our disposal. We manage to demonstrate that our new model is able to successfully take into consideration the context specified by the user. 
% Despite being limited by the computational resources at our disposal, we demonstrate that, using our pipeline, a small GPT2 model fine-tuned during only ten epochs on a few hundred of novels is able to successfully take into consideration the context specified by the user. 


==> _eval.tex <==
\subsection{Text generation framework}

We now want to generate text and evaluate the performance of our fine-tuned GPT-2LMHeadModel using the transformers library from Hugging Face\footnote{https://huggingface.co/transformers/}. In both evaluation and generation modes, the model input is of the form:
\begin{verbatim}
   [P3] P3 [Sum] Sum [T] Theme 
   [Ent] Entities [Size] 
   [P1] P1 [P2]
\end{verbatim}
Unlike in training, we do not input $P2$. Nevertheless, we need to leave sufficient space for it to be generated since the model's output is equal to the model's input plus the generated sequence. Hence, the input cannot exceed a certain limit, smaller than 1024 tokens, that we determine based on confidence intervals. If the input is too big, we truncate it, similarly to what was done in training.\\

In this mode, after encoding the input, we generate a proper new paragraph $P2$ using a carefully chosen decoding strategy, embedded in the transformers \textit{generate} function. More precisely, to generate a new word (or token), the model outputs a single vector and multiplies it by the learned embedding matrix. It yields an unique score for each word in the vocabulary, which determines ultimately the probability of each word to be generated. See Figure \ref{generation}. Choosing the best decoding strategy and hyperparameters is a key step to obtain a good generated text, as it has a big impact on the generation. Before delving into the main decoding strategies, remember that GPT-2 is an auto-regressive language generation model so 
\begin{equation*}
    P(w_{1:T} | Context) = \prod_{t=1}^T P(w_t | w_{1:t-1}, Context)
\end{equation*}
with $w_{0} = [P2]$. The length of the generated text is determined on the fly by the $<$eos$>$ token. It can however be controlled by a \textit{min\_length} and \textit{max\_length} parameter, that we use to bound the generation.

\noindent
Let's now develop the main decoding strategies.\\

\textbf{Greedy search}: $w_t = \arg \max_w P(w_t | w_{1:t-1})$. It is the most basic technique and consists in selecting the most probable word at each step in a greedy manner. \\

\textbf{Beam search} improves the greedy aspect of the model \cite{kulikov2019importance} by keeping the most likely \textit{num\_beams} hypotheses at each time step and eventually choosing the hypothesis that has the overall highest probability. It will always find an output sequence with higher probability than greedy search, but is not guaranteed to find the most likely output. Overall, it leads to a more fluent output but is often quite repetitive. It is particularly undesirable in story generation, even when corrected by \textit{repetition\_penalty} or \textit{no\_repeat\_ngram\_size}, which penalise repetitions \cite{yang2018breaking, holtzman2019curious}. \\ 

\textbf{Top-k sampling}: sampling  means randomly picking the next word according to the conditional distribution $w_t \sim P(w_t | w_{1:t-1})$. Lowering the temperature enables to sharpen the probability mass distribution. Increasing it fosters diversity and suits us better since we want creative outputs that give ideas to the writer, even if some mistakes are made. Top-k sampling builds on sampling, it simply selects the k most probable words and re-scales the probability mass distribution across the k selected words. This approach yields very nice results \cite{radford2019language}. Its sole limit is that k is fixed whether there is a narrow or wide distribution, while we might want to distinguish between those two cases. \\

\textbf{Nucleus sampling}: Instead of sampling only from the most likely k words, nucleus or top-p sampling chooses from the smallest possible set of words whose cumulative probability exceeds the probability p. The probability mass is then redistributed among this set of words. This way, the size of the set of words (a.k.a the number of words in the set) can dynamically increase and decrease according to the next word's probability distribution. Mathematically, we want to find $V^{(p)}$ the smallest set of words such that $\sum_{w \in V^{(p)}} P (w | w_{1:t-1}) \geq p $. This is the best approach so far \cite{holtzman2019curious} and is the one adopted by this paper, with $p=0.9$.\\

% Maybe recap final generation function parameters. + Give examples. 

\subsection{Evaluation}

We evaluate the final model, obtained after ten epochs of training, on a small portion of the training set and on some unseen novels. To do so, for each sample considered, we generate a new paragraph $P2$ and compare it with the true $P2$ by computing some carefully defined metrics (see below). Analysing them helps us determine if the model yields a more contextualised and controllable generation. Only one type of summary is used at once to generate $P2$ and consequently to assess the model. We thus perform an evaluation for each summarizer and especially focus on the two most representative ones: Keywords and BART, whose results are aggregated. \\
Coming back to the metrics utilised, we have implemented a few that we estimated relevant for this task, namely:\\


\textbf{Perplexity} to evaluate the fluency of the model. As a reminder, it gives a measure of how probable a sentence is to the model. We expect this metric to increase slightly compared to normal GPT-2 as better contextualisation often trades off with lesser fluency. This is computed using a non-fine-tuned GPT-2 model. \\

\textbf{Bert relationship} measures how the generated paragraph relates to its neighbouring paragraphs, how well it fits in. It indicates how our model deals with long contextualisation by computing the probability that $P3$ follows generated $P2$, normalised by the probability that $P3$ follows true $P2$. In practice, this metric outputs binary scores that are not very informative, so we do not include it in the results section. \\

\textbf{KwCount} and \textbf{EntitiesCount} respectively output the proportion of specified entities and the proportion of keywords\footnote{they are extracted from the summary of $P2$ if the Kw summarizer was not chosen for generation} actually appearing in the generated paragraph. It helps evaluate the control we have over the generation. \\

\textbf{BertSimilarity, Rouge} and \textbf{Bleu} give an indication of how close the generated P2 is to the true P2, meaning how well we reconstruct the initial paragraph. While Rouge uses n-grams overlap, Bleu regards precision and BertSimilarity the cosine similarity measure between their BERT [CLS] embeddings.


\subsection{Results}

\begin{figure*}[!t]
    \centering
    \includegraphics[width = 1 \textwidth]{Images/eval_sim_perplex.png}
    \caption{As foreseen, BertSimilarity (left) and Perplexity (right) are both higher for our model compared to raw GPT-2. BertSimilarity implies that an independent GPT-2 model considers our generations to be closer in a certain way to the original paragraphs, which is nice. Perplexity induces that the generated text is found less likely to appear and thus that our model is probably less fluent.}
    \label{eval_sim_perplex}
\end{figure*}

\begin{figure*}[!t]
    \centering
    \includegraphics[width = 1 \textwidth]{Images/eval_rouge_bleu.png}
    \caption{Rouge (left) and Bleu (right) scores: we see a small but significant increase of both metrics, meaning that the number of words and n-grams overlapping between original and generated P2 rises.}
    \label{eval_rouge_bleu}
\end{figure*}

\begin{figure*}[!t]
    \centering
    \includegraphics[width = 1 \textwidth]{Images/eval_entities_keywords.png}
    \caption{EntitiesCount (left) and KwCount (right). The graph shows that there is a significantly higher proportion of specified entities and keywords appearing in the generated text. However, without embedding this dimension into the loss function (penalise if omitted), we doubt that these statistics can improve much further.}
    \label{eval_entities_keywords}
\end{figure*}

To evaluate the model, we focus on the distribution of the above metrics across all paragraphs and compare our trained model with a raw GPT-2 model. Note that the overall performance of raw GPT-2 doesn't change whether we give it the full input (P1, P3, entities, keywords...) or only a reduced input like P1 (no context), as shown by appendix Figure \ref{append_rawgpt2}.

There are strong evidences that our model enables a greater control over the generated text. The proportion of specified entities (\textit{EntitiesCount}) and keywords (\textit{KwCount}) that we find in generated text is higher with our model than with GPT-2, as shown in Figure \ref{eval_entities_keywords}. This means that we are able to slightly steer the text generation according to authors' desires, including the elements they specify more often. Similarly, appendix Figure \ref{append_size} demonstrates that our model learns to adapt to the given paragraph size, without having to hard-code it in Hugging Face's \textit{generate}.

On a different note, the results demonstrated by \textit{BertSimilarity}, \textit{Rouge} and \textit{Bleu} (Figures \ref{eval_sim_perplex} and \ref{eval_rouge_bleu}) indicate that our model manages to reconstruct P2 better, confirming the trend perceived with the decreasing loss function (Figure \ref{loss}). 

Overall, our model seems to provide a more contextualised and controllable generation. The substantial improvement of all metrics compared to raw GPT-2 (with and without context information) suggests that our model learns to use the given context to generate new text, which is what we aspired to at the beginning. Nevertheless, as one could expect, this comes at the cost of a lower fluency, translated by a surge in the \textit{Perplexity} metric. 

Regarding human-assessed generation quality, it is difficult to truly observe it with our metrics, which is why we have made our model available to a group of authors and allowed them to play with it and share their results or impressions. Some generation samples can be found in the appendix. As you can notice there, generation quality is relatively poor. Although a bit disappointing, it was predictable as we are using a small GPT-2 model, whose results are far from the capabilities of GPT-2 Mega.

Finally, to grasp an idea of the evolution of the model performance, an evaluation at each epoch of the training was performed and is available in appendix Figure \ref{append_evolution}.


\subsection{Further developments}

An improvement we thought of consists in implementing a PPLM model on top of our fine-tuned GPT-2 model, in order to steer generation even further. We wanted to use it to control the sentiment of the text, the paragraph's theme or the genre of the book even better. However, despite yielding great results, PPLM only allows to customise generation according to six pre-defined themes and is therefore not of great help here.

From these results, we conclude that changing the loss function might be necessary to achieve greater control. Indeed, as we keep the cross-entropy unchanged, we have no direct control on the usage of the given context and simply hope that the network will use it to better reconstruct the original paragraph. We could try to add well-designed terms to the loss. For instance, terms that penalise the absence of an entity by looking at the output vector presenting the highest similarity with the entity's embedding. But it would require numerous iterations to be designed and tuned properly. 

Finally, taking a larger GPT-2 model (Large or Mega) would definitely produce much better texts and is probably necessary if we want our web-service to be truly useful to authors. Training the model on more samples (potentially less epochs) also seems promising as it would lead to a better generalisation.


==> _intro.tex <==

\subsection{Motivation}

The Transformer architecture \cite{vaswani1706attention} has enabled large scale language models trained on huge text corpora \cite{devlin2018bert, dai2019transformer} to improve significantly the state-of-the-art natural language processing. Regarding the specific task of text generation, OpenAI GPT-2 \cite{radford2019language} has reached outstanding performance and produces something close to what humans would write. However, it suffers from one major drawback: its output is not controllable. Steering generation thus has been the focus of some recent papers \cite{hu2017toward, logeswaran2018content}. Among the most successful, CTRL \cite{keskar2019ctrl} and PPLM \cite{dathathri2019plug} introduced respectively control codes and an attribute model to help govern style, theme and task specific behaviour. Others, like Grover \cite{zellers2019defending}, create fake news article using information about author, domain, data and headline. \\

These papers pave the way of future controllable text generation and demonstrate great possibilities. However, they show some limits; only a few definite features are controllable at once and user interaction remains restricted. Furthermore, despite being more accessible thanks to transfer learning, the lack of open source platforms and the difficulty to maintain a consistent context across long paragraphs have limited their spread towards day-to-day applications. \\

Being aware of such limitations, we join the recent trend of research papers that try to overcome these shortcomings. In particular, we wish to fill in a gap in the literature by building a tool aimed at helping an author write a novel. Our work can be decomposed into two steps. The main one being to find an original approach leading to a controllable and contextualised text generation, specific to novels. The second one being to integrate it into an interactive open-source web-service that allows any author to benefit from it. The code is available at \url{https://github.com/WeazelDev/AITextGenerator} and the front-end at \url{http://textgen.thomas-lamson.com/}. \\
% add interface link.

Our objective is to make users, at any point when writing a novel, able to automatically generate new sections that are consistent with the rest of the writing, especially previous and following paragraphs. We leave them the opportunity to select entities (characters, locations, etc.) that they have introduced in their novel and that they want to include in the new section. Similarly, they can specify the size of desired text, its content via a small summary or keywords and even the genre of the book they are writing. In the end, the tool we propose automatically makes several suggestions that users can choose from and edit. The objective being to produce creative outputs that give ideas to the writers while respecting the following constraints:
\begin{itemize}
\itemsep0em 
\item Ensure fluency and a correct syntax.
\item Consistently fill in the gap indicated by the author while conforming with surrounding context.
\item Respect the desired length and genre.
\item Use the selected entities and reflect the summary of the desired content. 
\end{itemize}


\subsection{Technical solution}

One issue here, as evoked in some papers, is the computational resources needed to train these big models \cite{shoeybi2019megatron, keskar2019ctrl}. Grover \cite{zellers2019defending} for instance, with its 1.5 billion parameters, required a training time of two weeks with 256 TPUs, which costed 35k\$. Due to our limited financial and computational resources, we were not able to train from scratch a powerful model that produces believable sentences. We were also unable to handle tremendous models endowed with billions of parameters, such as GPT-2 1.5B. \cite{radford2019language}.

In this paper, we fine-tune a GPT-2 117M model's parameters on 313 carefully pre-processed novels. We choose this model not only because it is one of the best text generators but also because it seems possible to contextualise the generation, despite being only a decoder. The latter is well illustrated by Hugging Face's conversational AI\footnote{https://github.com/huggingface/transfer-learning-conv-ai} and Gwern Branwen's GPT-2 Poetry\footnote{https://www.gwern.net/GPT-2}. \\

The general idea is pretty simple: usual text generation methods work by computing the probability distribution of the next word based on previous words \cite{siddharthan2002christopher, bengio2003neural}:
\begin{equation*}
    P(w_t | w_1, w_2, ..., w_{t-1})
\end{equation*} 

What we want to do is to condition this probability on a structured (theme, length of text, list of entities) and unstructured (content summary, previous and following paragraphs) context that will be specified by users. This yields: 
\begin{equation*}
    P(w_t | \textit{context}_{1:n}, w_{1:t-1})
\end{equation*}

This way, when computing the probability distribution for token $w_t$, GPT-2 model will have access to the context information established by users while our fine-tuning will have made it able to understand the input data format. \\

\noindent
In summary, our key \textbf{contributions} are: 
\begin{itemize}
\itemsep0em 
    \item Introduction of a novel GPT-2 fine-tuning approach for contextualised and controlled text generation.
    \item Results benchmark with original GPT-2 and examination of various metrics to quantify the effectiveness of our approach.
    \item Innovative User Interface (UI) ideas for a practical authored generation tool in an open-source JavaScript/Python web-service.
\end{itemize}

Finally, one of this paper's key characteristic is the integrated use of multiple models. Although the core generation is based on OpenAI GPT-2, we employ several other models like BERT, BART, T5, etc. (see next setion for references) at different steps of the project (data generation, new metrics, web-service). With this approach, we hope to inspire new cross-uses of such models in the field. 

==> _method.tex <==
\begin{figure*}[!t]
\includegraphics[width=1\textwidth]{Images/preproc.jpg}
\caption{Data Preprocessing Pipeline}
\label{preproc}
\end{figure*}

Before delving into the details of the process, let's make clear the intuition behind our approach. We train our model to re-generate each book's paragraph (called P2) using the previous and following paragraphs (P1 and P3) as well as information concerning P2: its size, the genre of the book it belongs to, the entities it showcases and a summary of its content. As evoked, we do not train a model from scratch but fine-tune a pre-trained GPT-2 model, teaching it to predict the next word using the above contextual information and already generated words. This helps our model learn how to generate paragraphs that are consistent with the provided context. Since it is trained on many books, it will hopefully be able to generalise and satisfy the objectives mentioned in the introduction. \\

Our approach is thus separated into three main steps. First, we create the appropriate database. Secondly, we transform and feed the data to GPT-2. Thirdly, we fine-tune the model.

\subsection{Data}
In this section, we emphasise some key aspects of the data generation phase since the contextualisation of the pre-trained GPT-2 strongly depends on it. \\

\textbf{Novels data}: Our paper focuses on text generation for novels and thus requires adequate data. We use the famous open book library Project Gutenberg\footnote{https://www.gutenberg.org/} to train our model. For each book existing on Gutenberg, we create a json file with its cleaned textual content and its related metadata: author, title, language, theme and genre. Note that a unique genre per book is manually defined from unstructured thematic information. It is the only metadata among those mentioned that we use for the fine-tuning and it is also exploited to filter the data. Indeed, we are interested and thus only keep books written in English and corresponding to a novel (using the genre tag). Although the process originally applies for all books on Gutenberg, we consider 500 of them due to limited computational resources and 313 are finally retained for training, after the filtering step. We then split the text of each book into paragraphs of different lengths, with a minimum and maximum bound, being careful not to cut a sentence in the middle, nor to separate core parts like chapters or even to split big paragraphs into uneven pieces. This step is essential as we will later learn to reconstruct them; the whole training builds on this split. Note that we store the size of each paragraph as a number of characters, which will then be used to categorise them as either \textit{Small},  \textit{Medium} or  \textit{Large}. \\

\textbf{Entity extraction}: Once each book is processed as detailed above, we detect entities for each paragraph using a pre-trained BERT NER Large model\footnote{https://github.com/kamalkraj/BERT-NER}. We sort them according to four categories: persons, locations, organisations and miscellaneous. Training the model with this data makes it capable of generating text that contains the established entities. It allows authors to specify the ones that they want to incorporate in the generation. \\

\textbf{Summary}: Similarly, in order for authors to be able to guide the generation by giving information on the desired content, we derive four very different summaries of each paragraph using state-of-the-art summarizers. Refer to the \textit{Related Work} section for more information on text summarization. \\
Using various summary types tends to make our model more robust to the possible ways authors could provide this type of information. Indeed, if users give the first sentence or a key sentence of the desired paragraph, extractive summarization via BertSum \cite{liu2019fine} will suit perfectly. On the other hand, if authors provide a detailed or brief summary of their idea, we will apply abstractive summarizers such as BART \cite{lewis2019bart} or T5 \cite{raffel2019exploring}, which have been fine-tuned differently to output texts of disparate lengths and employ distinct techniques. Finally, this paper incorporates a summarizer (denoted KW) that extracts keywords from the paragraph, allowing users to provide an unstructured sequence of words as a summary of the content \cite{mihalcea2004textrank}. It builds on graph theory as it constructs a word graph of the text based on co-occurence in a sliding window of size two. It then uses the pagerank centrality metric and POS tag to extract keywords from the word graph. \\

As a result, we obtain a json file per book containing the novel's related metadata (author, title, language, genre, theme) as well as the entire text split into paragraphs. Each of them comes with four different summaries (Bart, T5, BertSum, Kw) and a list of entities that appear in it. All entities and one summary chosen at random are fed to the GPT-2 model alongside metadata information (size and genre) and pure text (P1, P2, P3) to help it control and contextualise the generation. Figure \ref{preproc} illustrates this step. \\


\subsection{Preparation step}

\begin{figure*}[!t]
\includegraphics[width=1\textwidth]{Images/Training.jpg}
\caption{Training framework}
\label{training}
\end{figure*}

We distinguish training mode from evaluation and generation modes. This section is dedicated to the training mode only. \\
We want each datapoint to have the following form: 
\begin{verbatim}
   [P3] P3 [Sum] Sum [T] Theme 
   [Ent] Entities [Size] 
   [P1] P1 [P2] P2 <|endoftext|>
\end{verbatim}
where $[P1]$, $[P2]$, $[P3]$, $[Sum]$, $[T]$ and $[Ent]$ indicate the type of input received by the model (special tokens). $[Size]$ is slightly different as it can be any of $[S]$, $[M]$ or $[L]$ and gives information about the paragraph's length. The rest simply refers to the data stored in the json files and is easily accessible. Note that the order of the input is not essential. We only put $P1$ at the end so that GPT-2 can continue from there, as it has been trained to do so. \\

Usually, during training, GPT-2 takes as input an entire text file that it tokenizes and splits into blocks of size $=$ \textit{block\_size}, the maximum input size of the small GPT-2 model, 1024 tokens. It then keeps them in memory in a torch dataset and loads them through a dataloader. Quite obviously, we have to proceed differently here. We do not want to feed to GPT-2 a continuous text that would be split according to its maximum input capacity but instead the blocks that we specified above, one at a time. Since they would most probably not fill in perfectly GPT-2's input space, we pad on the right when necessary. When the input sample is too big, we truncate $P1$ on the left and $P3$ on the right, so as to stay around $P2$. This is not done evenly as we allocate $2/3$ of the remaining space\footnote{once everything except $P1$ and $P3$ has been fed as input} to $P1$ and $1/3$ to $P3$, as we consider $P1$ to be more important than P3.

Once we have the framework that formats the data that we would like to pass to the model, we tokenize it using GPT-2 Byte-Pair-Encoding (BPE) Tokenizer \cite{sennrich2015neural}. Note that we create special tokens for $[P1]$, $[P2]$, etc. This tokenized input of length $n$ has three different representations, all of shape $(1, n, 768)$ where $768$ is the embedding dimension for a small GPT-2, namely: 
\begin{enumerate}
    \item \textbf{Token embeddings}: vector representations of words, learned during training.
    \item \textbf{Positional embeddings}: vector representations (fixed or learned) that incorporate the sequential nature of the input, telling the model that words have a temporal property. They encode the position of a word in the input sentences.
    \item \textbf{Segment embeddings}: vector representations that help the model distinguish between the different segments of the input. They mark the segment to which each token belongs to. In this case, P1, P2, P3, theme, size, summary and entities.
\end{enumerate}
The network's input is in fact a single vector computed as the sum of the three embeddings above. We also give the network a label vector of dimension $(1,n,768)$ that equals $-100$ everywhere except for the tokens belonging to $P2$. This is ultimately used to compute the cross entropy loss function only between generated and original $P2$, token by token. Indeed, we do not train the model to reproduce the full input but only $P2$, our paragraph of interest, see \textbf{Figure \ref{training}}. The idea being that the model utilises the context information provided to learn a correct reconstruction of the paragraph of interest $P2$.  \\

\subsection{Fine tuning}

\begin{figure}
    \centering
    \includegraphics[width = 1 \linewidth]{Images/Loss fct.png}
    \caption{Loss function during training (smoothed)}
    \label{loss}
\end{figure}

We fine-tuned the pre-trained GPT2LMHeadModel (small) from hugging face, using a customised version of their training script. GPT2LMHeadModel is a GPT-2 model transformer with a language modelling head on top of it, that is a linear layer with weights tied to the input embeddings. Its documentation is available here\footnote{https://huggingface.co/transformers/model\_doc/GPT-2.html#} and detailed explanations about GPT-2 are accessible on the following blog \footnote{https://jalammar.github.io/illustrated-GPT-2/}. \\
We trained it on the 313 pre-processed books, using all of Hugging Face's training settings. As mentioned, we were limited in terms of resources and could not really run this project at a larger scale. Training was performed using CUDA on an AWS's p3.2xlarge instance (incorporating one NVidia Tesla V100 GPU) and costed about 150\$. In total, the model received 134k samples for each epoch, and there were 10 epochs. However, fewer epochs might be enough to reach great performances.



\begin{figure*}[!t]
\includegraphics[width=1\textwidth]{Images/generation.jpg}
\caption{Text generation process}
\label{generation}
\end{figure*}
 


==> _relatedwork.tex <==
\textbf{Language modelling}: The field of Natural Language Processing has undergone amazing progress in recent years, especially through language models \cite{bengio2003neural}. One key idea at the origin of this improvement consists in embedding the meaning of a particular word into a vector of scalars of chosen dimension \cite{mikolov2013efficient, pennington2014glove}. These word embeddings, or token embeddings, made it possible to perform a wide variety of tasks such as machine translation \cite{edunov2018understanding}, question-answering \cite{yang2019xlnet} or sentiment analysis \cite{radford2017learning} much better than existing statistics and grammar based approaches. In addition to reaching higher performances in the vast majority of tasks, it also started a new era of research. More recently, the use of the Transformer architecture \cite{vaswani1706attention} in some models like BERT \cite{devlin2018bert} revolutionised the field, improving dramatically our ability to capture the meaning of a word, a sentence or a document. Building on this, OpenAI described a transformer-decoder-only architecture focused on text generation: GPT-2 \cite{radford2019language}, which achieved outstanding performance. \\

\textbf{Controlled text generation}: Current state-of-art approaches for controlled text generation involve either training conditional generative models \cite{ficler2017controlling, keskar2019ctrl}, fine-tuning existing models with Reinforcement Learning \cite{ziegler2019fine} or training generative adversarial networks \cite{yu2017seqgan, zellers2019defending}. They yield high quality results but this comes at the expense of a huge training necessitating vast computational resources. To go around this, an even more recent approach, namely PPLM \cite{dathathri2019plug}, introduces a plug and play model that does not require retraining any conditional generative model. Similarly, our goal is conditional generation from a pre-trained unconditional model, avoiding big training needs. 
However, unlike them, we combine the large-scale pre-trained unconditional model, in this case OpenAI GPT-2, with a transfer learning fine-tuning technique. From this perspective, our work is similar to Hugging Face's state-of-the-art conversational AI\footnote{https://github.com/huggingface/transfer-learning-conv-ai} that contextualises dialog on both previous history and the bot's 'personality'.\\

\textbf{Interactive story telling}: Building on the above, some papers have chosen to explore controlled generation to assist story writing \cite{peng-etal-2018-towards, luo-etal-2019-learning}. In addition to research papers, a few open source websites like \textit{plot generator}\footnote{https://www.plot-generator.org.uk/story/} or \textit{talk to transformers}\footnote{https://talktotransformer.com/} generate stories where the author is sometimes asked to provide some context. It is nevertheless quite rudimentary. \textit{AI Dungeon}\footnote{https://aidungeon.io/} is maybe the only exception and their amazing work motivated us to conduct this research. All in all, our work greatly differs from theirs in its objectives. \\

\textbf{Text summarization}: It is the task of producing concise and fluent summaries while preserving key information content and overall meaning. Extractive summarization methods, like Refresh \cite{narayan-etal-2018-ranking} or BERT SUM \cite{liu2019fine}, which is a simple variant of BERT \cite{devlin2018bert}, returns specific passages of the document that are considered important. In contrast, abstractive summarization methods, like Pointer Generator Networks \cite{DBLP:journals/corr/SeeLM17} or UNIfied pre-trained Language Model \cite{dong2019unified}, generate a new text that conveys critical information from the original text. Although human summaries are abstractive, most research has been focused on extractive summarization until recently, when seq2seq framework with bidirectional encoder and left-to-right decoders such as BART \cite{lewis2019bart} and T5 \cite{raffel2019exploring}, have shown promising results. \\


==> _web.tex <==
During this project we also wanted to innovate and give a proposition of what an AI enhanced interface would look like in terms of user experience. We designed an interface and linked it to elastic instances in the back-end. We then opened it to a small public to test our model.\\

To gain in flexibility in the choice of instances to perform the heavy computations and to allow load balancing on several instances, we uncoupled the \textit{master} instance - serving the javascript front-end and general data - from the computational instances - performing NER and text generation on demand. It is also possible for the client to run the servers locally to avoid delays and server overloads. Figure \ref{web} gives an idea of the general architecture of our service. \\

\begin{figure}
    \centering
    \includegraphics[width = 1 \linewidth]{Images/web.png}
    \caption{Webservice architecture}
    \label{web}
\end{figure}

The front-end can be accessed at the following address: \url{http://textgen.thomas-lamson.com/}. The corresponding open-source code can be found on the github page: \url{https://github.com/WeazelDev/AITextGeneratorFront}. \\

In this interface, users are invited to write some text in a simple editor. Named entities like characters, locations, organisations and others are detected on the fly by the NER backend, and are displayed on the left panel. It is made easy for users to edit them manually if needed. \\

Users have the possibility to select several options: length of desired paragraph, genre of their writing and list of entities they want to see appear in the generation. They can also highlight a small part of the text that will act as a summary (or a list of keywords). When they are ready, they simply need to press the \textit{Generate} button and let the magic happen. 

